sparsegl: An R Package for Estimating Sparse Group Lasso

The sparse group lasso is a high-dimensional regression technique that is useful for problems whose predictors have a naturally grouped structure and where sparsity is encouraged at both the group and individual predictor level. In this paper we discuss a new R package for computing such regularized models. The intention is to provide highly optimized solution routines enabling analysis of very large datasets, especially in the context of sparse design matrices.

==> arxiv-sparsegl-preamble.tex <==
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\snorm}[1]{\lVert #1 \rVert}
\newcommand{\R}{\mathbb{R}}
\newcommand{\vbeta}{\boldsymbol\beta}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{y}}
\newcommand{\vy}{\vY}
\newcommand{\df}{\mathrm{df}}
\newcommand{\vR}{\mathbf{r}}
\newcommand{\Hessian}{\mathbf{H}}
\usepackage{amsmath, amsfonts, amsthm, amssymb}
\usepackage{algorithm, algorithmic}
\usepackage{nicefrac}
\usepackage{booktabs}
\usepackage[sort&compress,round]{natbib}
\usepackage[margin=1in]{geometry}
\usepackage{xcolor}
\renewcommand{\algorithmiccomment}[1]{\hfill $\rhd$ #1}
\def\algorithmautorefname{Algorithm}
\def\T{\mathsf{T}}

\usepackage[pagebackref=true]{hyperref}
\hypersetup{colorlinks=true,citecolor=blue,linkcolor=blue,urlcolor=blue}


\newtheorem{proposition}{Proposition}

\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\renewcommand*{\figureautorefname}{Figure}%
\renewcommand*{\tableautorefname}{Table}%
\renewcommand*{\sectionautorefname}{Section}%
\renewcommand*{\subsectionautorefname}{Section}%
\renewcommand*{\subsubsectionautorefname}{Section}%
%\usepackage{xcolor}
\newcommand\code{\bgroup\@makeother\_\@makeother\~\@makeother\$\@codex}
\def\@codex#1{{\normalfont\ttfamily\hyphenchar\font=-1 #1}\egroup}
\let\code=\texttt
\let\proglang=\textsf
\newcommand{\pkg}[1]{{\fontseries{m}\fontseries{b}\selectfont #1}}
\newcommand{\email}[1]{\href{mailto:#1}{\normalfont\texttt{#1}}}
%\ifx\csname urlstyle\endcsname\relax
%  \newcommand\@doi[1]{doi:\discretionary{}{}{}#1}\else
%  \newcommand\@doi{doi:\discretionary{}{}{}\begingroup
%\urlstyle{tt}\Url}\fi
%\newcommand{\doi}[1]{\href{https://doi.org/#1}{\normalfont\texttt{\@doi{#1}}}}

